Phoebe: A Learning-based Checkpoint Optimizer

Easy-to-use programming interfaces paired with cloud-scale processing engines have enabled big data system users to author arbitrarily complex analytical jobs over massive volumes of data. However, as the complexity and scale of analytical jobs increase, they encounter a number of unforeseen problems, hotspots with large intermediate data on temporary storage, longer job recovery time after failures, and worse query optimizer estimates being examples of issues that we are facing at Microsoft. To address these issues, we propose Phoebe, an efficient learning-based checkpoint optimizer. Given a set of constraints and an objective function at compile-time, Phoebe is able to determine the decomposition of job plans, and the optimal set of checkpoints to preserve their outputs to durable global storage. Phoebe consists of three machine learning predictors and one optimization module. For each stage of a job, Phoebe makes accurate predictions for: (1) the execution time, (2) the output size, and (3) the start/end time taking into account the inter-stage dependencies. Using these predictions, we formulate checkpoint optimization as an integer programming problem and propose a scalable heuristic algorithm that meets the latency requirement of the production environment. We demonstrate the effectiveness of Phoebe in production workloads, and show that we can free the temporary storage on hotspots by more than 70% and restart failed jobs 68% faster on average with minimum performance impact. Phoebe also illustrates that adding multiple sets of checkpoints is not cost-efficient, which dramatically reduces the complexity of the optimization.

==> Introduction.tex <==

\section{Introduction}
\label{sec:intro}

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.75\columnwidth]{trend3}
	\vspace{-0.6cm}
	\caption{Trends in \cosmos big data infrastructure at \msft show a significant increase in the volumes of data read and the number of tasks per analytical job.}\label{fig:trend}
	\vspace{-0.5cm}
\end{figure}


Big data platforms have democratized scalable data processing over the last decade, giving developers the freedom of writing complex programs (also referred to as \emph{jobs}) without worrying about scaling them~\cite{zaharia2010spark, thusoo2009hive,tigani2014google,chaiken2008scope,diaz2018azure,ramakrishnan2017azure,aws-athena, sarkar2018learning}. 
However, this flexibility has also led developers into building very large analytical programs that can put the underlying platform under stress.
For instance, the scale and flexibility of \textit{\cosmos}
~\cite{curino2019hydra,shao2019griffon,chaiken2008scope}, 
a big data analytics platform at \msft,
empower developers to author large jobs composed of pipelines of SQL-like query statements which are compiled into query plans composed of up to thousands of \emph{stages} (executable units composed by one or more operators) running over hundreds of thousands of processing units scheduled by YARN~\cite{vavilapalli2013apache}.
Figure~\ref{fig:trend} shows how the \cosmos workloads in one of the clusters have evolved over the past two years: we see that the 
total number of \emph{tasks} per job (each corresponding to one process executed in one container) have grown by $34\%$ (shown in blue), while the
volume of input data has grown by $80\%$ (shown in orange).
Large analytical jobs lead to several operational problems.

\stitle{Large jobs result in machine hotspots that run out of local storage space due to temporary data.} Big data systems typically persist intermediate outputs on local SSDs until the end of the query. However, large query plans end up consuming a substantial amount of temporary storage. 
To illustrate the problem, Figure~\ref{fig:ssd} (left) shows, for one \cosmos cluster, the cumulative distribution of available local SSD storage that is used for storing temporary data.
We can see that for different Stock Keeping Units (SKUs), $15-50\%$ of the machines run out of local storage on SSDs. %
This results in not only expensive spilling to HDDs and hence processing slowdown, but also an increase in incidents reporting job failures due to SSD outages. %
Currently, to avoid the SSD shortage, we need to either 
cap the number of containers running on each machine (thus wasting expensive CPU and memory resources)~\footnote{Alternate solution could be to make YARN scheduler aware of the SSD utilization. However, additional parameters are not only harder to tune cluster-wide but also increase the scheduling overhead, which could
translate into high costs at scale.}, or 
scale the CPU and memory together with the temporary storage in the newer SKUs.



\stitle{Large jobs are prone to longer re-starting time in case of failures.} 
Figure~\ref{fig:failure} (right) shows the failure rates of jobs with increasing runtimes. {\color{blue}We observe that even though a majority of the jobs finish within $20$ minutes, the failure rates in larger (> 100 minutes) jobs could range as high as $5\%$.} Network/communication failures, changes in cluster conditions, transient system behavior, and user errors are some of the common reasons for job failures in Cosmos.
Even though Cosmos already provides a lineage-based mechanism~\cite{rdd} for coping with task failures, improving resiliency to job failures and reducing recovery time are very important, especially as jobs and workloads scale.




\stitle{Large jobs end up having worse query optimizer estimates.} Errors in cardinality propagate exponentially~\cite{moerkotte2009preventing,neumann2013taking}, and hence complex jobs are more likely to produce poor query plans. A recent trend~\cite{rios,adptive-query-spark} suggests to re-optimize plans adaptively during job execution, but collecting statistics on-the-fly and on distributed intermediate results is highly not trivial and requires major overhaul of the runtime system.









\stitle{Checkpointing to the rescue.} Our observation is that the above problems can all be solved with a simple, yet effective technique: \textit{checkpointing intermediate state to a durable global storage}. In fact, by ``decomposing'' large jobs into smaller ones that are separated by persistent (e.g., with 3-way replication) checkpoints, 
we can (1) free up intermediate data on hotspots even before the job completes; (2) fast restart failed jobs from previous state; (3) collect statistics on the checkpoints and re-optimize large jobs into smaller ones with better estimates; and (4) reduce intermediate data in local storage to avoid wasting resources in newer SKUs.  
However, checkpointing is not free. It comes with I/O costs for moving intermediate data to durable global stores, storage costs on the global store, latency impact on the analytical job, and lack of debuggability because of intermediate data being cleared up. 
Furthermore, there are system challenges to transparently integrate checkpointing mechanism within the big data system.

In the literature, two types of checkpointing approaches are prominent. \textit{Runtime-based approaches} use information gathered at execution time to dynamically select when to checkpoint~\cite{daly2006higher,sharma2016flint,yan2016tr}. Runtime-based checkpointing requires gathering of statistics during execution as well as dynamic components which are not easily implementable in production systems such as Cosmos. 
Conversely, \textit{compile-time approaches} leverage information at the job level to propose optimal checkpoints to the system~\cite{upadhyaya2011latency,yang2010osprey,chen2013selective}.
This approach does not require any dynamic component and is therefore the solution we pick in this work. 
The challenge then is to select, efficiently and upfront, the set of intermediate data to checkpoint given a global storage budget.


\eat{

We evaluate some of those impacts in the production environment in this work.

In the literature, two types of checkpointing approaches are prominent. \textit{Runtime based approaches} use information gathered at execution time to dynamically select when to checkpoint~\cite{}. Conversely, \textit{compile-time based approacher} leverage information at the job level to proposal optimal checkpoint to the runtime~\cite{}.
In this work we 

\stitle{Challenges.}
The challenge, however, is to select the set of intermediate data to checkpoint given a global storage budget.

In this work, we demonstrate that a proactive {\it checkpoint} strategy at the compile time could help free up more than $70\%$ of the local storage on these hotspots and reduce the recovery time for these failed jobs by $64\%$ on average through proper modeling and optimization. However, note that checkpointing is not free; it comes with I/O costs for moving intermediate data to persistent stores, storage costs on the persistent store, latency impact on the analytical job, and lack of debuggability in case intermediate data is cleared up. We evaluate some of those impacts in the production environment in this work.
}

\begin{figure}[t]
	\centering
	\begin{minipage}[b]{0.5\columnwidth}
		\includegraphics[width=\textwidth]{trend5}
	\end{minipage}%
	\begin{minipage}[b]{0.5\columnwidth}
		\includegraphics[width=\textwidth]{failure}
	\end{minipage}%
	\vspace{-0.4cm}
	\caption{The Empirical Cumulative Density Function (ECDF) for SSD usage (left) and job failure rate with respect to job runtime and the probability density function (PDF) of job runtime distribution (right).}\label{fig:failure}\label{fig:ssd}
	\vspace{-0.6cm}
\end{figure}



\eat{
\begin{itemize}
	\item \textbf{The performance of checkpoint optimizer has to be very good to justify the action of flushing.} The solution of flushing to HDD can be costly due to the high expense of global storage on HDD. In the current implementation, the data in global storage will be replicated by three times and will not be deleted for a longer time, while the temp data storage used by a particular query job will always be cleared right after the query finishes. Therefore, it is desired that the optimizer is able to select the optimal set of checkpoints that maximizes the saving on temp data storage from the pre-checkpoint stages while using limited global storage.
	\item \textbf{Developing accurate cost models for the optimizer is a well-known difficult problem.} In the production environment, customer workloads may have significant different characteristics with various User Defined Operators (UDOs), and the noisy neighbors on the same server affect the latency dramatically. To estimate the potential saving/usage for the storage, the detailed execution schedule (starting time and ending time) and the output size of each stage are required as inputs, which
	is well-known a challenging task
	given limited information about the query and its input data at the compiling time.
	\item \textbf{There are various practical concerns for the deployment of such pipeline in production.} (i) Integration: in the analyzed system, we rarely have any ML-based application that is applied at a large scale at the compiling time. Therefore, the detailed design on the model training and deployment pipeline is critical. (ii) Latency: in the production system, the ML training and testing pipelines should be with low latency with respect to the frequency needed for retraining. The optimization should be also solved with low latency at the compiling time. (iii) Data quality: there are data quality issues that need to be properly addressed.
\end{itemize}
}

\stitle{Introducing Phoebe.}
In this paper, we present Phoebe: a learning-based checkpointing optimizer for determining, at the compile-time, the decomposition (or the ``cuts'') of large job 
graphs in big data workloads.
{\color{blue}
Phoebe addressed the following key challenges. (1) Implementing an efficient checkpointing framework requires accurate estimates of the cardinalities of jobs. However, cardinality estimates are often off by several orders of magnitudes~\cite{dutt2019selectivity,MCSN,siddiqui2020cost}, and even learned approaches are good for relative plan comparisons~\cite{marcus2019plan,marcus2019neo,ortiz2018learning}, while they lack in absolute terms.
(2) Previous checkpointing approaches are mostly effective on relatively small tree-shaped plans; conversely SCOPE jobs are complex Direct Acyclic Graphs (DAGs) composed by up to several thousand operators and several hours long runtimes.
(3) To optimize the return of investment, a checkpointing solution must be applicable in different scenarios (as described above) and be flexible enough to adapt to different objective and constraints, while still thriving for optimality. 

To solve the above challenges, Phoebe advances the state of the art on several front. First, Phoebe is build upon state-of-the-art cost models, i.e., CLEO~\cite{siddiqui2020cost} (which has improved the default SCOPE cost model by orders of magnitude), and use its operator-level estimation as featurizer, automatically capturing, for each operator, workload characteristics. Given that our focus is on recurrent jobs, and that majority of the workloads for \cosmos are recurrent (>70\%), Phoebe leverages historical statistics (such as average) from previous runs as additional features to the estimators. 
By mixing historical with plan features, Phoebe is able generate cardinality estimates, and as we will see in our experimental evaluation, Phoebe can reach better accuracy compared to state-of-the-art approaches (i.e., CLEO). 
Second, in Phoebe we make the important observation that to get the most benefits from a compile-time checkpointing solution, both stage output sizes and scheduling (i.e., start/end times) information are required. 
This is because cardinality estimates are not enough to estimate the actual storage cost, since they don't take into account for how long the data need to be persisted. 
Since intermediate output data must be saved on temporary data storage locally till the end of the job, Phoebe proposes a Time-to-Live (TTL) estimator for the lifetime of the temporary data, and that takes into account the full execution runtime of the job.
Third, to our knowledge, Phoebe is the first checkpointing framework that considers multiple objectives (constraints) in the optimization problem. 
Existing checkpoint optimization mechanisms only focus on one dimension, such as minimizing runtime overheads~\cite{daly2006higher,sharma2016flint,upadhyaya2011latency}, or rely on brute-force algorithms to search for the optimal solution~\cite{chen2013selective,salama2015cost,yang2010osprey}. 
In SCOPE, a brute force approach is a no starter given the tight SLAs and large DAGs, while in this paper, we propose a flexible solution whereby directive objectives can be used to pick the optimal checkpoint.
}
\eat{
{\color{blue}The checkpoint mechanism of Cosmos is implemented at the {\it stage-level}\footnote{A stage consists of a set of operators physically executing on the same machine.} and with explicit capacity constraints for the global storage (which is more costly) where the output of checkpoint stages will be stored. Stage-level predictors developed in Phoebe turn out to be highly accurate since they train on metrics from physically executed tasks with explicit materialization boundaries. 
They also do not suffer from the exponential propagation of prediction errors, as seen in traditional cardinality estimation~\cite{moerkotte2009preventing,neumann2013taking}.

The core methodological contribution in Phoebe are two-fold.

First, for the cost estimators, to evaluate the potential benefits of the checkpointing solution in the optimizer, detailed information of stage output sizes and scheduling (i.e., start/end times) is required. Specifically, the intermediate output data will be saved on temp data storage locally till the end of the job. For the application of saving temp data storage, a Time-to-Live (TTL) estimator for the lifetime of the temp data is needed that takes into account the full execution process of the job. Compared with cardinality estimation to be used as input to the query optimizer (e.g.,~\cite{marcus2019plan,marcus2019neo,ortiz2018learning}), the estimation for TTL is more challenging as it requires always to consider the full execution plan, as oppose to a sub-tree. And the accuracy requirement is higher as most of the cardinality estimation only requires to have the same relative order for the estimation of different plans. For SCOPE~\cite{chaiken2008scope,zhou2012scope} jobs that have large and complex query plans, the estimation for the cost is even more challenging due to error prorogation issues~\cite{moerkotte2009preventing, salama2015cost,neumann2013taking}. In this paper, we propose a plethora of innovative ideas to achieve the best accuracy:
\begin{itemize}
\item We build upon a state-of-the-art cost model for SCOPE jobs, i.e., CLEO~\cite{siddiqui2020cost} (which has improved the default SCOPE cost model by orders of magnitude), and use its operator-level estimation as input that automatically captures workload characteristics such as Input Cardinality, AverageRowLength, and Number of Partitions, for each operator. 

\item Given that majority of the workloads for \cosmos are recurrent (>70\%), we leverage historical statistics from previous runs as one of the input to the estimator and only consider recurrent jobs for checkpointing. The analysis shows that it is the combination of historical statistics, and job-instance features that leads to better accuracy.
Table~\ref{table:job} shows the average and coefficient of variance (CV, defined by the ratio of standard deviation to the average) of data size and runtime for 5 job templates. We can see that for some jobs, the variation of runtime and data read/write is large (with CV>1). Therefore, a good predictor should both consider the historic statistics, and job-instance features.

\aj{could we say we are instance optimizing operator-level models with stage-level physical execution time in the workload telemetry?}

\begin{table}[t]
	\caption{{\color{blue}Example of Recurrent Job Templates}}\label{table:job}
	\begin{tabular}{lllllll}
		\toprule
		& \multicolumn{2}{l}{Job Runtime (s)} & \multicolumn{2}{l}{Data Read (byte)} & \multicolumn{2}{l}{Data Write (byte)} \\
		& Average            & CV            & Average             & CV            & Average             & CV             \\\midrule
		Job A & 240.54             & 1.17           & 1.01E+11            & 2.01           & 8.42E+10            & 1.93            \\
		Job B & 65.79              & 0.10           & 3.66E+06            & 1.95           & 1.46E+07            & 1.96            \\
		Job C & 6848.13            & 1.92           & 1.68E+13            & 0.94           & 5.18E+12            & 1.84            \\
		Job D & 749.58             & 0.52           & 1.96E+13            & 0.53           & 1.00E+10            & 0.53            \\
		Job E & 44.65            & 0.16           & 412            & 0           & 412            & 0       \\
		\bottomrule    
	\end{tabular}
\end{table}
\item Compared to prior work that focus on much simpler query plans~\cite{marcus2019plan, marcus2019neo,ortiz2018learning,mou2016convolutional,MCSN,akdere2012learning}, a SCOPE job can easily have hundreds or thousands of stages and hours' long execution time. The existing Deep Neural Net (DNN) solutions (e.g.,~\cite{MCSN,DBLP,marcus2019neo,NeuroCard,mou2016convolutional,marcus2019plan,ortiz2018learning}) are not applicable for large query plans due to the nature of gradient descend algorithm that are used in the training process. And the error prorogation issue for most of the existing cost models~\cite{moerkotte2009preventing, salama2015cost,neumann2013taking} renders them inapplicable. In this work, we propose an explainable simulation process given the stage-level cost that has proved to have better accuracy for large jobs. A detailed comparison of the cost estimation accuracy from CLEO and Phoebe is shown in Section~\ref{sec:result}.
\end{itemize}



Second, this paper is the first to efficiently considers multiple dimensions of constraints/objectives in the checkpoint optimizer, such as the trade-off of using the more costly global storage versus the storage saving for temp data, or the corresponding recovery time saving. A checkpoint optimization problem is typically formulated as a graph optimization problem, where stages on the the ``frontier''of the lineage graph~\cite{sharma2016flint,yang2010osprey} will be checked\footnote{{\color{blue}The decision is made at the compile time instead of during the runtime of the job, while the latter still requires dynamic decision making modules and cost estimators.}}. Existing checkpoint optimization mechanisms only focus on one dimension, such as minimizing runtime overheads~\cite{daly2006higher,sharma2016flint,upadhyaya2011latency}, which is a way simpler problem, or rely on brutal-force algorithms to inefficiently search for the optimal solution~\cite{chen2013selective,salama2015cost,yang2010osprey}. In this paper, we explicitly consider the storage cost (both in size and time dimensions) and the trade-off for using more expensive global storage and provides an efficient algorithm for solving it. 
	}}
In fact, we are able to run Phoebe at Cosmos-scale and our results show that 
Phoebe can free more than $70\%$ of the local storage on hotspots, and reduce the recovery time for failed jobs by $64\%$ on average, while increasing job latency by less than 3\%. %

{\color{blue}To summarize:
\begin{itemize}
 \item We introduce Phoebe: a system for making checkpoint decisions over big data workloads that leverages past workloads and makes checkpointing predictions for future queries;
 \item Phoebe learns accurate stage-wise predictors for stage-output size stage-runtime and stage-output TTL; 
 \item  We introduce a scalable checkpoint optimization algorithm for large query DAGs and global constraints over hundreds of thousands of jobs; and
	\item We evaluate the approach over production workloads, and show how the various components contribute towards picking good checkpoints as well as the involved trade-offs. 
\end{itemize}
}



The remainder of this paper is organized as follows. Section~\ref{sec:motivation} provides the background on Cosmos and SCOPE. Section~\ref{sec:overview} presents the end-to-end architecture. Section~\ref{sec:module1} describes the stage-level cost models for runtime and output size, while Section~\ref{sec:ttl} discusses the time-to-live estimator used for predicting the scheduling of stages. Section~\ref{sec:opt} discusses the checkpoint optimizer. Section~\ref{sec:result} presents the experiment results in the production environment. The paper ends with related work in Section~\ref{sec:related} and conclusions in Section~\ref{sec:conclude}.




